The Tags Are Alright: Robust Large-Scale RFID Clone Detection Through Federated Data-Augmented Radio Fingerprinting

Millions of RFID tags are pervasively used all around the globe to inexpensively identify a wide variety of everyday-use objects. One of the key issues of RFID is that tags cannot use energy-hungry cryptography. For this reason, radio fingerprinting (RFP) is a compelling approach that leverages the unique imperfections in the tag's wireless circuitry to achieve large-scale RFID clone detection. Recent work, however, has unveiled that time-varying channel conditions can significantly decrease the accuracy of the RFP process. We propose the first large-scale investigation into RFP of RFID tags with dynamic channel conditions. Specifically, we perform a massive data collection campaign on a testbed composed by 200 off-the-shelf identical RFID tags and a software-defined radio (SDR) tag reader. We collect data with different tag-reader distances in an over-the-air configuration. To emulate implanted RFID tags, we also collect data with two different kinds of porcine meat inserted between the tag and the reader. We use this rich dataset to train and test several convolutional neural network (CNN)--based classifiers in a variety of channel conditions. Our investigation reveals that training and testing on different channel conditions drastically degrades the classifier's accuracy. For this reason, we propose a novel training framework based on federated machine learning (FML) and data augmentation (DAG) to boost the accuracy. Extensive experimental results indicate that (i) our FML approach improves accuracy by up to 48%; (ii) our DA approach improves the FML performance by up to 31%. To the best of our knowledge, this is the first paper experimentally demonstrating the efficacy of FML and DA on a large device population. We are sharing with the research community our fully-labeled 200-GB RFID waveform dataset, the entirety of our code and trained models.

==> appoggio_grafici.tex <==
\begin{figure}[t]
    \centering
    \captionsetup{justification=centering}
    \begin{subfigure}[t]{0.31\columnwidth}
    \centering
    \setlength\fwidth{.6\columnwidth}
    \setlength\fheight{0.5\columnwidth}
    \input{./latex_figs/diagonal_24_beam_tm_0_l_1}
    \caption{24-beam, TX Ant. 0 \\Accuracy: 81.84\%}
    \label{fig:beam_pattern_24_atn_0}
    \end{subfigure}
    \begin{subfigure}[t]{0.31\columnwidth}
    \centering
    \setlength\fwidth{.6\columnwidth}
    \setlength\fheight{0.5\columnwidth}
    \input{./latex_figs/diagonal_12_beam_tm_0_l_1}
    \caption{12-beam, TX Ant. 0\\Accuracy: 80.89\%}
    \label{fig:beam_pattern_12_ant_0}
    \end{subfigure}
    \begin{subfigure}[t]{0.31\columnwidth}
    \centering
    \setlength\fwidth{.6\columnwidth}
    \setlength\fheight{0.5\columnwidth}
    \input{./latex_figs/diagonal_aoa_tm_0_l_1}
    \caption{AoA, RX Ant. 0\\Accuracy: 92.95\%}
    \label{fig:beam_pattern_aoa_ant_0}
    \end{subfigure}
    %
    % \begin{subfigure}[t]{0.31\columnwidth}
    % \centering
    % \setlength\fwidth{.6\columnwidth}
    % \setlength\fheight{0.5\columnwidth}
    % \input{./latex_figs/obstacle_24_beam_tm_0_l_1}
    % \caption{24-beam, TX Ant. 0\\Accuracy: 84.69\%}
    % \label{fig:beam_pattern_24_ant_0Obst}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.31\columnwidth}
    % \centering
    % \setlength\fwidth{.6\columnwidth}
    % \setlength\fheight{0.5\columnwidth}
    % \input{./latex_figs/obstacle_12_beam_tm_0_l_1}
    % \caption{12-beam, TX Ant. 0\\Accuracy: 84.41\%}
    % \label{fig:beam_pattern_12_ant_0Obst}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.31\columnwidth}
    % \centering
    % \setlength\fwidth{.6\columnwidth}
    % \setlength\fheight{0.5\columnwidth}
    % \input{./latex_figs/obstacle_aoa_tm_0_l_1}
    % \caption{AoA, RX Ant. 0\\Accuracy: 88.13\%}
    % \label{fig:beam_pattern_aoa_ant_0_obst}
    % \end{subfigure}
        \setlength\belowcaptionskip{-.5cm}
    \caption{Diagonal and Obstacle Results.}
        \label{fig:diagonal_obstacle}
\end{figure}


\begin{figure}[t]
    \centering
    \captionsetup{justification=centering}
    \begin{subfigure}[t]{0.44\columnwidth}
    \centering
    \setlength\fwidth{.6\columnwidth}
    \setlength\fheight{0.5\columnwidth}
    \input{./latex_figs/tAvA}
    \caption{T a V a \\Accuracy: 89.33\%}
    \label{fig:beam_pattern_24_atn_0}
    \end{subfigure}
    \begin{subfigure}[t]{0.44\columnwidth}
    \centering
    \setlength\fwidth{.6\columnwidth}
    \setlength\fheight{0.5\columnwidth}
    \input{./latex_figs/tBvB}
    \caption{T b V b\\Accuracy: 84.49\%}
    \label{fig:beam_pattern_12_ant_0}
    \end{subfigure}
       \centering
    \captionsetup{justification=centering}
    \begin{subfigure}[t]{0.31\columnwidth}
    \centering
    \setlength\fwidth{.6\columnwidth}
    \setlength\fheight{0.5\columnwidth}
    \input{./latex_figs/tABvA}
    \caption{T ab V a \\Accuracy: 93.11\%}
    \label{fig:beam_pattern_24_atn_0}
    \end{subfigure}
    \begin{subfigure}[t]{0.31\columnwidth}
    \centering
    \setlength\fwidth{.6\columnwidth}
    \setlength\fheight{0.5\columnwidth}
    \input{./latex_figs/tABvB}
    \caption{T ab V b\\Accuracy: 94.84\%}
    \label{fig:beam_pattern_12_ant_0}
    \end{subfigure}
       \centering
    \captionsetup{justification=centering}
    \begin{subfigure}[t]{0.31\columnwidth}
    \centering
    \setlength\fwidth{.6\columnwidth}
    \setlength\fheight{0.5\columnwidth}
    \input{./latex_figs/tABvAB}
    \caption{T ab V ab \\Accuracy: 93.97\%}
    \label{fig:beam_pattern_24_atn_0}
    \end{subfigure}
  
    
    %
    % \begin{subfigure}[t]{0.31\columnwidth}
    % \centering
    % \setlength\fwidth{.6\columnwidth}
    % \setlength\fheight{0.5\columnwidth}
    % \input{./latex_figs/obstacle_24_beam_tm_0_l_1}
    % \caption{24-beam, TX Ant. 0\\Accuracy: 84.69\%}
    % \label{fig:beam_pattern_24_ant_0Obst}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.31\columnwidth}
    % \centering
    % \setlength\fwidth{.6\columnwidth}
    % \setlength\fheight{0.5\columnwidth}
    % \input{./latex_figs/obstacle_12_beam_tm_0_l_1}
    % \caption{12-beam, TX Ant. 0\\Accuracy: 84.41\%}
    % \label{fig:beam_pattern_12_ant_0Obst}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.31\columnwidth}
    % \centering
    % \setlength\fwidth{.6\columnwidth}
    % \setlength\fheight{0.5\columnwidth}
    % \input{./latex_figs/obstacle_aoa_tm_0_l_1}
    % \caption{AoA, RX Ant. 0\\Accuracy: 88.13\%}
    % \label{fig:beam_pattern_aoa_ant_0_obst}
    % \end{subfigure}
        \setlength\belowcaptionskip{-.5cm}
    \caption{Diagonal and Obstacle Results.}
        \label{fig:diagonal_obstacle}
\end{figure}


==> img/results/cm-all/cmall.tex <==
\begin{tikzpicture}
\pgfplotsset{every tick label/.append style={font=\tiny}}

\begin{axis}[
enlargelimits=false,
colorbar,
colormap/Purples,
width=\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
tick align=inside,
xlabel={Train Set},
xmin=-0.5,
xmax=6.5,
xtick style={draw=none},
xtick = {0,1,2,3,4,5,6},
xticklabels = {OTA20,OTA50,OTA100,PM0-20,PM1-20,PM0-50,PM1-50},
xlabel style={font=\scriptsize\color{white!15!black}},
ylabel style={font=\scriptsize\color{white!15!black}},
ylabel={Test Set},
ymin=-0.5,
ymax=6.5,
xlabel shift=-5pt,
ylabel shift=-5pt,
ytick style={draw=none},
ytick = {0,1,2,3,4,5,6},
yticklabels = {OTA20,OTA50,OTA100,PM0-20,PM1-20,PM0-50,PM1-50},
axis background/.style={fill=white},
xticklabel style = {rotate=45,anchor=east},
colorbar horizontal,
colorbar style={
at={(0,1.05)},               % <-- (changed)
anchor=below south west,    % <-- (changed)
% change the width of the colorbar relative to the main `axis' environment
width=\pgfkeysvalueof{/pgfplots/parent axis width},
xtick={0, 0.5, 1},
xmin=0,
xmax=1,
axis x line*=top,
xticklabel shift=-1pt,
point meta min=0,
point meta max=1,
},
colorbar/width=2mm,
]\addplot [matrix plot,point meta=explicit]
 coordinates {
(0,0) [0.805191134977836] (0,1) [0.05509973666165741] (0,2) [0.001166707416009723] (0,3) [0.05944215065257555] (0,4) [0.0] (0,5) [0.046439048231321285] (0,6) [0.03266122206059998] 

(1,0) [0.07192173483121793] (1,1) [0.7747331837365004] (1,2) [0.077713667632193] (1,3) [0.01605528276413074] (1,4) [0.017960517811038208] (1,5) [0.0027535277810029923] (1,6) [0.0388620854439166] 

(2,0) [0.07898955644865033] (2,1) [0.05448606935396333] (2,2) [0.7079213008695214] (2,3) [0.028735493415597183] (2,4) [0.01969474302410467] (2,5) [0.03464129634785029] (2,6) [0.0755315405403129] 

(3,0) [0.035255754032421226] (3,1) [0.07174495319118653] (3,2) [0.0026118006220879385] (3,3) [0.7411869631126164] (3,4) [0.03949488053662497] (3,5) [0.0659406945478594] (3,6) [0.04376495395720359] 

(4,0) [0.011785504270030419] (4,1) [0.039026448645579796] (4,2) [0.04754141349893379] (4,3) [0.10628879021827067] (4,4) [0.7679421494316813] (4,5) [0.0006642436841433443] (4,6) [0.026751450251360675] 

(5,0) [0.05706311638600783] (5,1) [0.07923360075362468] (5,2) [0.0026617942768758928] (5,3) [0.07147696950156951] (5,4) [0.0053171558619136] (5,5) [0.7824377079983589] (5,6) [0.0018096552216496067] 

(6,0) [0.046605965523989976] (6,1) [0.0] (6,2) [0.06870261273158942] (6,3) [0.024828410957547276] (6,4) [0.05020402493255895] (6,5) [0.0001467172237318132] (6,6) [0.8095122686305826] 


};
\node[text=white] at (axis cs: 0,0) {\scriptsize 96\%};
\node[text=white] at (axis cs: 1,1) {\scriptsize 97\%};
\node[text=white] at (axis cs: 2,2) {\scriptsize 94\%};
\node[text=white] at (axis cs: 3,3) {\scriptsize 95\%};
\node[text=white] at (axis cs: 4,4) {\scriptsize 98\%};
\node[text=white] at (axis cs: 5,5) {\scriptsize 99\%};
\node[text=white] at (axis cs: 6,6) {\scriptsize 98\%};
\end{axis}
\end{tikzpicture}

%%0,96	0,97	0,94	0,95	0,98	0,99	0,98
